Optimal Accounting of Differential Privacy via Characteristic Function

Characterizing the privacy degradation over compositions, i.e., privacy accounting, is a fundamental topic in differential privacy (DP) with many applications to differentially private machine learning and federated learning. We propose a unification of recent advances (Renyi DP, privacy profiles, $f$-DP and the PLD formalism) via the \emph{characteristic function} ($\phi$-function) of a certain \emph{dominating} privacy loss random variable. We show that our approach allows \emph{natural} adaptive composition like Renyi DP, provides \emph{exactly tight} privacy accounting like PLD, and can be (often \emph{losslessly}) converted to privacy profile and $f$-DP, thus providing $(\epsilon,\delta)$-DP guarantees and interpretable tradeoff functions. Algorithmically, we propose an \emph{analytical Fourier accountant} that represents the \emph{complex} logarithm of $\phi$-functions symbolically and uses Gaussian quadrature for numerical computation. On several popular DP mechanisms and their subsampled counterparts, we demonstrate the flexibility and tightness of our approach in theory and experiments.

==> adv_joint_conv_proof.tex <==

Our proof of Theorem~\ref{thm:amplification_by_sampling} is based on the results of \citep{balle2018couplings}. In particular, the they have proven the following lemma about Hockey stick divergences known as the ``Advanced joint convexity'' which is very convenient for us.
\begin{lemma}[Advanced joint convexity {\citep[Theorem 2]{balle2018couplings}}]\label{lem:adv_joint_convex}
	Let $\mu,\nu,\nu'$ be three probability distributions (that are absolutely continuous w.r.t. the same base measure). 
	Let $\alpha'  =  1+\gamma(\alpha - 1)$ and $\beta = \alpha' / \alpha$. Then for all $\alpha \geq 0,  0 \leq \gamma \leq 1$, 
	$$
	H_{\alpha'}((1-\gamma)\mu + \gamma \nu \| (1-\gamma)\mu + \gamma \nu')  =  \gamma  H_{\alpha}(\nu \|  (1-\beta)\mu + \beta \nu').
	$$
	where $(1-\gamma)\mu + \gamma \nu$ denotes the mixture distribution of $\mu$ and $\nu$ (as the same convenient abuse of notation as before).
\end{lemma}
\begin{proof}
	We note that the range of parameter $\alpha$ is extended from $\alpha\geq 1$ to $\alpha > 0$. It is easy to verify that the same proof from \citep[Theorem 2]{balle2018couplings} works without changes.  
	
	For the case when $\alpha <1$, we have $1> \alpha'>\alpha$ and the above statement $(1-\beta)\mu + \beta \nu'$ may no longer be a probability distribution (because some elements might be negative).
	This is the reason the original theorem was stated only for $\alpha \geq 1$. However, for $\alpha<1$, $H_{\alpha}(\nu \|  (1-\beta)\mu + \beta \nu')$ can still be well-defined as  follows
	$$
	H_{\alpha}(\nu \|  (1-\beta)\mu + \beta \nu') :=  \int (\nu - ((\alpha-\alpha')\mu + \alpha'\nu' ))_+ 
	$$
	for all $\alpha>0$ and can be extended to the case when $\alpha=0$ by taking the limit.	Notice that $\alpha\beta = \alpha'$ and $\alpha(1-\beta)=\alpha-\alpha'$.  By the definition of  $\alpha$ and $\alpha'$,  it is easy to check that by plugging in $\alpha = 1 + (\alpha'-1)/\gamma$
	\begin{align*} 
		\gamma\int (\nu - ((\alpha-\alpha')\mu + \alpha'\nu' ))_+  &=  \int (\gamma\nu + (1-\gamma)\mu - \big((1-\gamma)-\gamma(\alpha-\alpha')\big)\mu   - \alpha'\gamma\nu' )_+    \\
		&=\int (\gamma\nu + (1-\gamma)\mu - \alpha'(1-\gamma)\mu   - \alpha'\gamma\nu' )_+  = H_{\alpha'}((1-\gamma)\mu + \gamma \nu \| (1-\gamma)\mu + \gamma \nu').
		\end{align*}
\end{proof}

\[
	H_{\alpha'}((1-\gamma)\mu + \gamma \nu \| \nu)  =  \gamma  H_{\alpha}(\mu \|\nu).
\]


\begin{proof}[Proof of Theorem~\ref{thm:amplification_by_sampling}]
We first consider the ``Removal'' neighboring relation, i.e., $|D| = |D'| +  1$.  w.l.o.g. assume $|D| = n+1$ and  the first $n$ data point are shared. Recall that Poisson sampling includes each individual data point with probability $\gamma$ independently, thus $\mathcal{M}(D)$ and $\mathcal{M}(D')$ are mixture distributions indexed by these Bernoulli random variables. Let $\cI$ be the indicator vector denoting the realized inclusion of the first $n$ data points and $J$ to denote the inclusion of the $(n+1)$th data point for $D$.
Denote $F =:\mathcal{M}\circ S_{\textbf{Poisson}} (D)$ and $G:=\mathcal{M} \circ S_{\textbf{Poisson}} (D')) $ and their density being $f,g$:
\begin{align*}
	H_{\alpha'}(F\|G) &=\int_o\left( \sum_{\cI} \pi(\cI) f(o| \cI) - \alpha' \sum_{\cI} \pi(\cI) g(o| \cI) \right)_+  do\\
	&\leq \int_o  \sum_{\cI} \pi(\cI)  ( f(o| \cI) - \alpha' g(o| \cI) )_+  do\\
	&=\sum_{\cI} \pi(\cI)   \int_o   ( f(o| \cI) - \alpha' g(o| \cI) )_+  do\\
	&=\sum_{\cI} \pi(\cI)   H_{\alpha'}( (1-\gamma)\mathcal{M}(D_{\cI}) + \gamma \mathcal{M}(D_{\cI \cap \cJ}) \| \mathcal{M}(D_{\cI}) ).
	%H_{\alpha}( \mathcal{M}((1-\gamma)\mu + \gamma \nu\|(1-\gamma)\mu + \gamma \nu')  
\end{align*}


Condition on $\cI$ and denote $\mu := \mathcal{M}(D_{\cI})$, $\nu := \mathcal{M}(D_{\cI\cap \cJ})$ as short hands for the density (or mass) functions.  

Let $\alpha := 1 + \frac{\alpha'-1}{\gamma}$, such that $\alpha'  =  1+\gamma(\alpha - 1)$ and define $\beta = \alpha' / \alpha$, by advanced joint convexity (Lemma~\ref{lem:adv_joint_convex}), we have
\begin{align*}
	H_{\alpha'}((1-\gamma)\mu + \gamma \nu\|\mu  )  &=  \gamma  H_{\alpha}(\nu \|  (1-\beta)\mu + \beta \mu) = \gamma  H_{\alpha}(\nu \|  \mu)\\ 
	&\leq \gamma H_{\alpha}(P \|Q ) = H_{\alpha'}((1-\gamma)Q + \gamma P\|Q  ) 
\end{align*}
where the inequality follows from that $(P,Q)$ is a dominating pair for $\mathcal{M}$ in the ``removal'' neighboring relation and the last identity follows by applying the advanced joint convexity backwards.
%	where the inequality follows because $(1-\alpha\beta)  = 1-\alpha'\leq 1$ and  $\alpha\frac{1-\beta}{1-\alpha\beta} \geq  \alpha$ (which implies that$H_{\alpha\frac{1-\beta}{1-\alpha\beta}}(\nu\|\mu)\leq H_{\alpha}(\nu\|\mu)$ by the fact that $H_{\alpha}$ is monotonic decreasing in $\alpha$. ) 

In the case when  $|D| = |D'| -  1$, w.l.o.g. assume $|D|=n$ and $D$ is identical to the first $n$ data points in $D'$.  By a similar argument we can get 
$$
H_{\alpha'}(F\|G) \leq \sum_{\cI} \pi(\cI) H_{\alpha'}(\mathcal{M}(D_{\cI}) \|(1-\gamma) \mathcal{M}(D'_{\cI}) + \gamma \mathcal{M}(D'_{\cI\cup \cJ}))
$$
Denote short hands $\mu:=\mathcal{M}(D_{\cI})  = \mathcal{M}(D'_{\cI}) $ and $\nu:=\mathcal{M}(D'_{\cI\cup\cJ})$, by advanced joint convexity
\begin{align*}
	H_{\alpha'}(\mu\|(1-\gamma)\mu + \gamma \nu )  &=  \gamma  H_{\alpha}(\mu \|  (1-\beta)\mu + \beta \nu) = \gamma \int ( (1-\alpha + \alpha')\mu  - \alpha'\nu )_+.
\end{align*}
When $(1-\alpha + \alpha')>0$, the above is equal to
$$
\gamma(1-\alpha + \alpha')H_{\frac{\alpha'}{1-\alpha + \alpha'}}(\mu\|\nu) \leq \gamma(1-\alpha + \alpha')H_{\frac{\alpha'}{1-\alpha + \alpha'}}(P\|Q) = H_{\alpha'}(P\|(1-\gamma)P + \gamma Q ).
$$
where we applied the definition of dominating pair for ``Addition''-neighboring relation  and roll back the identity.

When $(1-\alpha + \alpha')\leq 0$
$$
\gamma \int ( (1-\alpha + \alpha')\mu  - \alpha'\nu )_+ = 0 =  \gamma \int ( (1-\alpha + \alpha')P  - \alpha'Q)_+ = H_{\alpha'}(P\|(1-\gamma)P + \gamma Q ),
$$
where we know that for any $P,Q$ the above is true, therefore the dominating pair works.
\end{proof}

\begin{comment}
\begin{proof}[Proof of Theorem~\ref{thm:amplification_by_sampling}]
	The proof rely on the ``advanced joint-convexity'' property of  (see Lemma~\ref{lem:adv_joint_convex}).
	By Theorem 8 of \citep{balle2018couplings}, we know that for any  $D \simeq_{\textbf{add/remove}} D'$
	\begin{align*}
	&H_{e^\epsilon}(\cM\circ S_{\textbf{Poisson}}^\gamma(D) \| \cM\circ S_{\textbf{Poisson}}^\gamma(D')) \leq \gamma \sup_{\tilde{D}\simeq_{\text{add/remove}} \tilde{D}'} H_{1 + \frac{e^\epsilon-1}{\gamma}}(\cM(\tilde{D})\|\cM(\tilde{D}'))  \\
	\leq&  \gamma H_{1 + \frac{e^\epsilon-1}{\gamma}}(P\|Q)  = \gamma H_{1 + \frac{e^\epsilon-1}{\gamma}}(P\|\beta Q + (1-\beta) Q)\\
	=&H_{e^\epsilon}((1-\gamma)Q + \gamma P \| (1-\gamma) Q + \gamma Q) = H_{e^\epsilon}((1-\gamma)Q + \gamma P \|  Q).
	\end{align*}
	where the inequality in the second line is due to that $(P,Q)$ is a dominating pair of $\cM$, and the last line follows from the  advanced joint-convexity lemma when we choose $\beta = \frac{1+\gamma (e^\epsilon-1)}{e^\epsilon}$. Finally, observe that the bound holds for all $\epsilon\geq 0$.
	
	The same proof works line by line for the random subset sampling when we use Theorem 9  of \citep{balle2018couplings} instead and adopt the $D \simeq_{\textbf{swap}} D'$ neighboring relationship.
\end{proof}
\end{comment}

==> subsample.tex <==
\section{Subsample Mechanisms}\label{sec: subsample}
% the structure
% why we consider subsample? Which subsample mechanisms that we consider?
% How to identify the worst-case pair? 
		% Hocky-stick divergence can be used to identify the worst-case pair
		% Then we can write the privacy loss RV for the worst-case pair
% what if we do not have a closed-form expression？

A prime use case for the tight privacy accounting is the \textit{NoisySGD} algorithm~\cite{song2013stochastic, abadi2016deep}, which first takes a subset generated through some subsampling procedure, and then applies the gaussian mechanism on the subsampled data points. Here we consider two popular subsampling methods, Poisson subsampling and sampling with a fixed size subset.


\begin{description}
	\item[Poisson Sampling] Denoted by $S_{\textbf{Poisson}}$. $S_{\textbf{Poisson}}$ takes a dataset of size $n>0$ and return a dataset by including data point $i\in \{1,2,...,n\}$ with probability $0\leq \gamma \leq 1$ i.i.d. at random.
	\item[Subsampling]  Denoted by $S_{\textbf{Subset}}$. $S_{\textbf{Subset}}$ takes a dataset of size $n>0$ and return a subset of size $m \leq n$  uniformly at random.  We denote $\gamma := m / n$ for convenience. 
\end{description}

In DP analysis, it is essential to identify the worst-case pair of the neighboring dataset, which might be straightforward for basic mechanisms (take the datasets that attain the global sensitivity), but it is more challenging for advanced mechanisms.  Concretely, in subsampling, the output distribution $P = \cM \circ S_{\textbf{Subset}(D)}$ and $Q = \cM \circ S_{\textbf{Subset}(D')}$ are two mixture distributions over all possible combinations of within the chosen subset. Without specifying the worst-case pair of the neighboring dataset, the privacy loss RV expression can be messy, which can potentially lead to an intricate and lossy privacy analysis. One of our contributions is, we identify the worst-case pair of distributions for subsampled mechanisms, which not only simplifies our following analysis but also improves over the previous results on privacy amplification by subsampling (see Remark~\ref{rem: rdp}).
%To find the worst-pair $D, D'$ that attains the max $\delta$ in the privacy profile,  we need to take into account all possible combinations within the choosen subset. 
% say it's one of our contribution
\subsection{Worst-case pair of distributions for subsampled mechanisms}
Recall that identifying the worst-case pair of distribution is equivalent to identifying the dataset that attains the max $\delta$ in the Hockey-stick divergence. Moreover, the Hockey stick divergence also satisfies an identity known as the ``Advanced joint convexity,'' which is convenient for us.
\begin{lemma}[Advanced joint convexity {\citep[Theorem 2]{balle2018couplings}}]\label{lem:adv_joint_convex_main}
	Let $\mu,\nu,\nu'$ be three probability distributions (that are absolutely continuous w.r.t. the same base measure). 
	Let $\alpha'  =  \gamma(\alpha - 1)$ and $\beta = \alpha' / \alpha$. Then for all $\alpha \geq 1,  0 \leq \gamma \leq 1$, 
	$$
	H_{\alpha'}((1-\gamma)\mu + \gamma \nu \| (1-\gamma)\mu + \gamma \nu')  =  \gamma  H_{\alpha}(\nu \|  (1-\beta)\mu + \beta \nu').
	$$
	where $(1-\gamma)\mu + \gamma \nu$ denotes the mixture distribution of $\mu$ and $\nu$ (as the same convenient abuse of notation as before).
\end{lemma}


\begin{lemma}[Poisson sampled mechanisms] \label{lem:poisson_sample_main}
	Let $\cM$ be a randomized algorithm (that can take any sized data set). Let $D,D'$ be any two neighboring datasets where $|D| = |D'| +  1$.	 For all $\epsilon \geq 0$,
	\begin{align*}
&H_{e^\epsilon}(\cM\circ S_{\textbf{Poisson}} (D)\|\cM \circ S_{\textbf{Poisson}} (D')) \\
	& \leq   \sup_{\tilde{D} \sim_{\text{Add/Remove}} \tilde{D'} }    H_{e^\epsilon}( (1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D'})\| \cM(\tilde{D}) )
   \end{align*}
	where we abused the notation to use $(1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D'})$ to denote that distribution induced by a randomized mechanism that outputs $\cM(\tilde{D})$ with probability $\gamma$ and $\cM(\tilde{D}')$ with probability $1-\gamma$.
	The same conclusion also states when $|D|=|D'|-1$\yq{}{I change this part}
	%In the case when $|D| = |D'| - 1$,   for all $\epsilon \geq 0$,
	%\begin{align*}
	%&H_{e^\epsilon}(\cM\circ S_{\textbf{Poisson}} (D)\|\cM \circ S_{\textbf{Poisson}}(D'))\\
	 % &\leq   \sup_{\tilde{D} \sim_{\text{Add/Remove}} \tilde{D'} } H_{e^\epsilon}(\cM(\tilde{D}) \| (1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D'})).
	%\end{align*}
	
\end{lemma}

Next we combine the above lemmas and the ``Advanced joint convexity'' to prove the following new result about subsampled mechanisms.
\begin{lemma}[Subsampled mechanisms]\label{lem:subsample_main}
	Let $\cM$ be a randomized algorithm (that takes datasets of size $m$). Let $D,D'$ be any two  datasets that are identical to each other except on one of the data points.	 For all $\epsilon \geq 0$,
	\begin{align*}
	 &H_{e^\epsilon}(\cM\circ S_{\textbf{Subset}} (D)\|\cM \circ S_{\textbf{Subset}} (D')) \\
	 &\leq   \sup_{\tilde{D} \sim_{\text{Swap}} \tilde{D'} }    H_{e^\epsilon}( (1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D'})\| \cM(\tilde{D}) ).
	\end{align*}
	%	$$
	%	\sup_{\substack{ \tilde{D} \sim_{\text{swap}} \tilde{D}' \\
	%	\tilde{D} \sim_{\text{swap}} \tilde{D}''\\
	%\tilde{D'} \sim_{\text{swap}} \tilde{D''}}	}    H_{e^\epsilon}( (1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D'})\| (1-\gamma)\cM(\tilde{D}) + \gamma \cM(\tilde{D}'')).
	%	$$
	and that the RHS is maximizes by the pair of datasets that attains $\sup_{\tilde{D} \sim_{\text{Swap}} \tilde{D'} } H_{1 + \frac{e^{\epsilon}}{\gamma}}(\cM(\tilde{D}) \| \cM(\tilde{D'}))$.
\end{lemma}

\begin{remark}[Exact optimality of the bounds]
	For some $\cM$ mechanisms, there are datasets such that the inequalities in Lemma~\ref{lem:poisson_sample} and Lemma~\ref{lem:subsample} take $=$.  For example, consider $\cM$ to be Gaussian mechanism (or Laplace mechanism) that releases the total the number of $1$ in a dataset.  Then two neighboring datasets $D = [0,...,0,0]$, $D' = [0,0,...,0,1]$ exactly matches the bounds.
\end{remark}
\begin{remark}[Worst-case pair of distributions for sampled mechanisms]
	Lemma~\ref{lem:poisson_sample_main} and Lemma~\ref{lem:subsample_main}  also imply that when  there is a fixed pair $(D,D')$ that attains the max $\delta$ given all $\epsilon \geq 0$ in $\cM$ then there is a fixed pair of distributions $P,Q$  that attains the max $\delta$ given all $\epsilon \geq 0$ in $\cM \circ S_{subset}$ and $\cM \circ S_{Poisson}$ too.
	
	Specifically, for the interest of obtaining $(\epsilon,\delta)$-DP of the subsampled mechanism,  it suffices to consider two specific distributions: $P = (1-\gamma)\cM(D) + \gamma \cM(D')$ and $Q = \cM(D')$ and prove that 
	$$
	P(o \in S) \leq e^\epsilon Q(o\in S) + \delta
	$$
	for all $S\subset \cO$.   
\end{remark}
\begin{remark}[Renyi DP and Optimal Moments Accountant for subsampled mechanisms]\label{rem: rdp}
Renyi-DP and moments accountant are closely related concepts that are often considered identical. However, our results suggest that there is a distinction.  The above pair of $P,Q$ we constructed are not necessarily attaining the Renyi-DP bounds (see a concrete example from~\cite{zhu2019poission}, but as moments accountant focuses only on computing $(\epsilon,\delta)$-DP, it suffices use the Renyi-divergence functions $R_{\alpha}(P\|Q)$.    Specifically, this closes the constant gap between the moments accountant for subsampled mechanisms and Poisson sampled mechanisms.
\end{remark}

\subsection{Poisson subsampling}

The discussion above allows us to consider the following one dimension distribution as the worst-case pair neighboring distribution for the Poisson subsampling Gaussian mechanism.
\begin{align*}
	p(o) &= \gamma \frac{1}{\sqrt{2\pi \sigma^2}}e^{\frac{(o-1)^2}{-2\sigma^2}} + (1-\gamma)\frac{1}{\sqrt{2\pi \sigma^2}}e^{\frac{o^2}{-2\sigma^2}}\\
	q(o)&= \frac{1}{\sqrt{2\pi \sigma^2}}e^{\frac{o^2}{-2\sigma^2}}
\end{align*}
Therefore, the pairing privacy loss RV is given by
$$
L_{D,D'} = \log \bigg(\gamma e^{\frac{2y-1}{2\sigma^2}}+1-\gamma\bigg),  L_{D',D}= -\log \bigg(\gamma e^{\frac{2y-1}{2\sigma^2}}+1-\gamma \bigg) 
$$

At first glance, the privacy loss distribution above is complicated, which might not have a closed-form expression for the characteristic function. Thus, we choose to apply the discretization method to approximate the Poisson subsampling.  

We set $S = 100$ and $N=10^5$ to discretize the exact integral of $o$, which is $[-\infty, \infty]$ for the Gaussian mechanism. We use $\gamma=0.01$ and $\sigma \in \{1.0, 2.0\}$, for number of compositions up to $8000$.  Our method is compared to the RDP accountant described in~\citet{zhu2019poission}.



